Expectation consistency for calibration of neural networks

Despite their incredible performance, it is well reported that deep neural networks tend to be overoptimistic about their prediction confidence. Finding effective and efficient calibration methods for neural networks is therefore an important endeavour towards better uncertainty quantification in deep learning. In this manuscript, we introduce a novel calibration technique named expectation consistency (EC), consisting of a post-training rescaling of the last layer weights by enforcing that the average validation confidence coincides with the average proportion of correct labels. First, we show that the EC method achieves similar calibration performance to temperature scaling (TS) across different neural network architectures and data sets, all while requiring similar validation samples and computational resources. However, we argue that EC provides a principled method grounded on a Bayesian optimality principle known as the Nishimori identity. Next, we provide an asymptotic characterization of both TS and EC in a synthetic setting and show that their performance crucially depends on the target function. In particular, we discuss examples where EC significantly outperforms TS.

==> affine_teacher/affine_teacher_relative_difference.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figheight,
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Relative difference  \(\displaystyle \Delta T / T_{TS}\)},
ymajorgrids,
ymin=0.00808263786168649, ymax=0.0964984507680401,
ytick style={color=black}
]
\addplot [draw=color0, fill=color0, mark=*, only marks, scatter]
table{%
x  y
1 0.0151363400958749
1.48717948717949 0.0172331756099838
1.97435897435897 0.0222356804952378
2.46153846153846 0.0224727115425563
2.94871794871795 0.0281892908673519
3.43589743589744 0.0296033229676535
3.92307692307692 0.0365267580156714
4.41025641025641 0.0375634008702857
4.8974358974359 0.0427630485411347
5.38461538461538 0.04510895919007
5.87179487179487 0.050021950224639
6.35897435897436 0.0537510511575162
6.84615384615385 0.0594367514596314
7.33333333333333 0.0564066226174101
7.82051282051282 0.0583786624113146
8.30769230769231 0.0605871768377172
8.7948717948718 0.064800428411621
9.28205128205128 0.0726423714443663
9.76923076923077 0.0633617045961618
10.2564102564103 0.0744575954156312
10.7435897435897 0.0706509958257595
11.2307692307692 0.0745546628069746
11.7179487179487 0.0712424154475891
12.2051282051282 0.0815938790619494
12.6923076923077 0.07987986112762
13.1794871794872 0.0824586075292515
13.6666666666667 0.0790033553624058
14.1538461538462 0.0838680449378904
14.6410256410256 0.0821531535458041
15.1282051282051 0.0854658647685055
15.6153846153846 0.0834152946739423
16.1025641025641 0.0823812347089928
16.5897435897436 0.0863892943395045
17.0769230769231 0.0887356436159343
17.5641025641026 0.0886554112502323
18.0512820512821 0.0882474100291704
18.5384615384615 0.0888728715995087
19.025641025641 0.0907672797259036
19.5128205128205 0.089844256132683
20 0.0924795501813877
};
\addplot [semithick, color0]
table {%
1 0.0121015384483389
1.48717948717949 0.0159600383446919
1.97435897435897 0.0191379697770742
2.46153846153846 0.0218273914421418
2.94871794871795 0.0242399284918305
3.43589743589744 0.0270653901277244
3.92307692307692 0.0337562329349698
4.41025641025641 0.0393238758215561
4.8974358974359 0.0438338267196012
5.38461538461538 0.0477204032964127
5.87179487179487 0.051165773594923
6.35897435897436 0.0542587352227779
6.84615384615385 0.0570852418020452
7.33333333333333 0.0596505475625118
7.82051282051282 0.0620363275491453
8.30769230769231 0.0642206437942322
8.7948717948718 0.0662326425029536
9.28205128205128 0.0681187046076588
9.76923076923077 0.0698773201033472
10.2564102564103 0.0715159347105361
10.7435897435897 0.0730407700015985
11.2307692307692 0.0744731146815771
11.7179487179487 0.0758332949223246
12.2051282051282 0.0770873412677037
12.6923076923077 0.0782941007393231
13.1794871794872 0.0794204349156341
13.6666666666667 0.0804866868669766
14.1538461538462 0.0814965093681872
14.6410256410256 0.0824545121858343
15.1282051282051 0.0833701093790081
15.6153846153846 0.0842398556085927
16.1025641025641 0.0850568541334762
16.5897435897436 0.0858451648127864
17.0769230769231 0.0865707636992444
17.5641025641026 0.0872894891576945
18.0512820512821 0.0879731410865527
18.5384615384615 0.0886248284415442
19.025641025641 0.089237879519549
19.5128205128205 0.0898340761906901
20 0.0904058617632092
};
\end{axis}

\end{tikzpicture}


==> constant_teacher/constant_teacher_relative_difference.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.647058823529412,0}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Relative difference  \(\displaystyle \Delta T / T_{TS}\)},
ymajorgrids,
ymin=-0.00130000246447956, ymax=0.303553453348903,
ytick style={color=black}
]
\addplot [draw=color0, fill=color0, forget plot, mark=*, only marks, scatter]
table{%
x  y
1 0.0156359335601499
1.48717948717949 0.0125569727997651
1.97435897435897 0.024722736211889
2.46153846153846 0.0270668866741009
2.94871794871795 0.0403460127481245
3.43589743589744 0.0341715704259338
3.92307692307692 0.0766364811595017
4.41025641025641 0.088671818131378
4.8974358974359 0.119626485217223
5.38461538461538 0.10012117111977
5.87179487179487 0.128211157409077
6.35897435897436 0.106384226513938
6.84615384615385 0.126680284698584
7.33333333333333 0.130126344766854
7.82051282051282 0.138637360633119
8.30769230769231 0.140640026493109
8.7948717948718 0.171459662755168
9.28205128205128 0.158991963470476
9.76923076923077 0.180785312127454
10.2564102564103 0.172381646859328
10.7435897435897 0.168272990915476
11.2307692307692 0.192660002325984
11.7179487179487 0.192450266435639
12.2051282051282 0.201839230626814
12.6923076923077 0.211749005300134
13.1794871794872 0.206411711595742
13.6666666666667 0.215771394740272
14.1538461538462 0.195467857424946
14.6410256410256 0.231796320874372
15.1282051282051 0.236815406251558
15.6153846153846 0.246719260711447
16.1025641025641 0.256777404911938
16.5897435897436 0.245652444085573
17.0769230769231 0.224028783229418
17.5641025641026 0.288434989860511
18.0512820512821 0.261818118713328
18.5384615384615 0.266998126403211
19.025641025641 0.289696478084658
19.5128205128205 0.266643089629938
20 0.258647666721105
};
\addplot [semithick, color0]
table {%
1 0.0127140893391908
1.48717948717949 0.0167927874416053
1.97435897435897 0.0203033734226291
2.46153846153846 0.027070757971925
2.94871794871795 0.0429792801127694
3.43589743589744 0.0557869808616585
3.92307692307692 0.0675170526820274
4.41025641025641 0.0785768206936381
4.8974358974359 0.0891212245840087
5.38461538461538 0.099198969861594
5.87179487179487 0.108854850928242
6.35897435897436 0.118108934352487
6.84615384615385 0.127010632678464
7.33333333333333 0.135536364731892
7.82051282051282 0.143738994055264
8.30769230769231 0.151607764854664
8.7948717948718 0.15916601936948
9.28205128205128 0.166452129517935
9.76923076923077 0.173435209952785
10.2564102564103 0.180147663568115
10.7435897435897 0.186599686689499
11.2307692307692 0.192812702474115
11.7179487179487 0.198769910141708
12.2051282051282 0.204510831406729
12.6923076923077 0.210050533888488
13.1794871794872 0.215371228032846
13.6666666666667 0.220494103120885
14.1538461538462 0.225437667321066
14.6410256410256 0.230179144935238
15.1282051282051 0.234758825369641
15.6153846153846 0.239169712926581
16.1025641025641 0.243424700395972
16.5897435897436 0.247529763623118
17.0769230769231 0.251492039611132
17.5641025641026 0.255319182320396
18.0512820512821 0.259018099119162
18.5384615384615 0.262570394203155
19.025641025641 0.26601579791989
19.5128205128205 0.269344895606136
20 0.272579607023013
};
\addlegendentry{$\sigma_{CONST}$}
\end{axis}

\end{tikzpicture}


==> logit_teacher/logit_teacher_relative_difference.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figheight,
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Relative difference  \(\displaystyle \Delta T / T_{TS}\)},
ymajorgrids,
ymin=0.00038490210650353, ymax=0.00208156507914493,
ytick style={color=black}
]
\addplot [draw=color0, fill=color0, mark=*, only marks, scatter]
table{%
x  y
1 0.000462023150714503
1.48717948717949 0.000602470093450275
1.97435897435897 0.000809277667252931
2.46153846153846 0.00121151856437121
2.94871794871795 0.00148509442251603
3.43589743589744 0.00150379077436698
3.92307692307692 0.00174345553337398
4.41025641025641 0.00190894518958171
4.8974358974359 0.0019427440471961
5.38461538461538 0.00179804565430677
5.87179487179487 0.00197873926395673
6.35897435897436 0.00198700708936501
6.84615384615385 0.00200444403493396
7.33333333333333 0.00199972430209456
7.82051282051282 0.00200000185184167
8.30769230769231 0.00190563835105904
8.7948717948718 0.0019023209792755
9.28205128205128 0.00195209581057124
9.76923076923077 0.00196308754279534
10.2564102564103 0.00184626217103798
10.7435897435897 0.00184756017439881
11.2307692307692 0.00182430003276102
11.7179487179487 0.00178382104814397
12.2051282051282 0.00183252553936068
12.6923076923077 0.00173862162413878
13.1794871794872 0.00188066094503442
13.6666666666667 0.00174355690968924
14.1538461538462 0.00168621316200239
14.6410256410256 0.00175553334967942
15.1282051282051 0.00171353098965743
15.6153846153846 0.00156028623576021
16.1025641025641 0.0017585991331515
16.5897435897436 0.00180168550720455
17.0769230769231 0.00151835487188877
17.5641025641026 0.00153122778474199
18.0512820512821 0.00167011001454102
18.5384615384615 0.00142231031017206
19.025641025641 0.00138845133092015
19.5128205128205 0.00150543908662474
20 0.00148839920131915
};
\addplot [semithick, color0]
table {%
1 0.000589988634129368
1.48717948717949 0.000708293705587901
1.97435897435897 0.000789964136126098
2.46153846153846 0.001098228616311
2.94871794871795 0.00140589933023946
3.43589743589744 0.00159943873245626
3.92307692307692 0.00173668273838204
4.41025641025641 0.00182986815393864
4.8974358974359 0.00189443987386998
5.38461538461538 0.00193775950681515
5.87179487179487 0.00197484306400807
6.35897435897436 0.00198390556938507
6.84615384615385 0.00200247613826795
7.33333333333333 0.00199956410536413
7.82051282051282 0.00199476719269664
8.30769230769231 0.00198560088678506
8.7948717948718 0.00197806079720671
9.28205128205128 0.00195526915171475
9.76923076923077 0.00193480348411761
10.2564102564103 0.00191223752558322
10.7435897435897 0.0018918638811322
11.2307692307692 0.00187167064545975
11.7179487179487 0.00184795191882112
12.2051282051282 0.00182888223736288
12.6923076923077 0.00180047809070184
13.1794871794872 0.00177348564779448
13.6666666666667 0.00176897851038554
14.1538461538462 0.00174443552656251
14.6410256410256 0.0017202057058638
15.1282051282051 0.00169622046516174
15.6153846153846 0.00167254566766779
16.1025641025641 0.00164857249604391
16.5897435897436 0.00162405692698497
17.0769230769231 0.00160299566577993
17.5641025641026 0.00158723470411071
18.0512820512821 0.00155571386972682
18.5384615384615 0.00154709710135647
19.025641025641 0.0015077449621815
19.5128205128205 0.00149978722023299
20 0.00148024056246153
};
\end{axis}

\end{tikzpicture}


==> real_data/resnet20_0.9_calibration.tex <==

% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
 \usetikzlibrary{patterns}
 \tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=0.5, xmax=1,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.5,0) rectangle (axis cs:0.583333333333333,0.41082164645195);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.5};
\addlegendentry{TS & EC}

\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.583333333333333,0) rectangle (axis cs:0.666666666666667,0.556179761886597);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.666666666666667,0) rectangle (axis cs:0.75,0.654285728931427);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.75,0) rectangle (axis cs:0.833333333333333,0.735632181167603);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.833333333333333,0) rectangle (axis cs:0.916666666666667,0.834545433521271);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.916666666666667,0) rectangle (axis cs:1,0.974084317684174);
\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.5,0) rectangle (axis cs:0.583333333333333,0.337719291448593);
\addlegendimage{ybar,ybar legend,draw=black,postaction={pattern=north east lines}};
\addlegendentry{Uncalibrated}

\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.583333333333333,0) rectangle (axis cs:0.666666666666667,0.478632479906082);
\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.666666666666667,0) rectangle (axis cs:0.75,0.526923060417175);
\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.75,0) rectangle (axis cs:0.833333333333333,0.597173154354095);
\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.833333333333333,0) rectangle (axis cs:0.916666666666667,0.717616558074951);
\draw[draw=black,postaction={pattern=north east lines}] (axis cs:0.916666666666667,0) rectangle (axis cs:1,0.938621878623962);
\addplot [semithick, black, dashed, forget plot]
table {%
0.5 0.5
1 1
};
\end{axis}

\end{tikzpicture}


==> rho_10/logistic_teacher_rho_10_relative_difference.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figheight,
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Relative difference  \(\displaystyle \Delta T / T_{TS}\)},
ymajorgrids,
ymin=2.30855768561792e-05, ymax=0.00167498568625423,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
1 9.81719454651816e-05
1.48717948717949 0.000125919851488869
1.97435897435897 0.000167909873681575
2.46153846153846 0.000230894348369137
2.94871794871795 0.000298094646070899
3.43589743589744 0.000363711057243521
3.92307692307692 0.000426943425494069
4.41025641025641 0.000487401976256296
4.8974358974359 0.000545330402722595
5.38461538461538 0.000600772592776288
5.87179487179487 0.000653938645171882
6.35897435897436 0.000704920787925107
6.84615384615385 0.000753919518746628
7.33333333333333 0.000801059380196913
7.82051282051282 0.000846377556269742
8.30769230769231 0.000889977932213823
8.7948717948718 0.000931968600990532
9.28205128205128 0.000972500201512625
9.76923076923077 0.00101161831059369
10.2564102564103 0.00104933792828903
10.7435897435897 0.00108587142326827
11.2307692307692 0.00112096756932471
11.7179487179487 0.00115504840152914
12.2051282051282 0.00118796380152566
12.6923076923077 0.00121980874538348
13.1794871794872 0.00125073605807154
13.6666666666667 0.00128070624509093
14.1538461538462 0.00130974342220396
14.6410256410256 0.00133793912353138
15.1282051282051 0.0013652501489994
15.6153846153846 0.00139166850980572
16.1025641025641 0.00141752591344812
16.5897435897436 0.00144258923548529
17.0769230769231 0.00146698831233364
17.5641025641026 0.00149063685188626
18.0512820512821 0.00151362610080567
18.5384615384615 0.00153610917376004
19.025641025641 0.00155784618849174
19.5128205128205 0.0015791483839447
20 0.00159989931764523
};
\end{axis}

\end{tikzpicture}


==> rho_10/logit_teacher_rho_10_ece.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{1,0.647058823529412,0}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=0.0499999999999999, xmax=20.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={ECE},
ymajorgrids,
ymin=0.00555449302000508, ymax=0.0294213768331223,
ytick style={color=black}
]
\addplot [semithick, blue]
table {%
1 0.00663935137514677
1.48717948717949 0.00753079039758812
1.97435897435897 0.00870944049481127
2.46153846153846 0.0102325569498806
2.94871794871795 0.0116538488241866
3.43589743589744 0.0129029895326343
3.92307692307692 0.014007848177021
4.41025641025641 0.0149978975868902
4.8974358974359 0.0158952313349759
5.38461538461538 0.016716041316785
5.87179487179487 0.0174724310858538
6.35897435897436 0.0181736892925857
6.84615384615385 0.0188271150057693
7.33333333333333 0.0194385683283043
7.82051282051282 0.0200128403382279
8.30769230769231 0.0205539061153254
8.7948717948718 0.0210651083510688
9.28205128205128 0.0215492892574929
9.76923076923077 0.0220088928038758
10.2564102564103 0.0224460379745065
10.7435897435897 0.0228625707796551
11.2307692307692 0.0232601256637702
11.7179487179487 0.0236401328799886
12.2051282051282 0.0240038783164817
12.6923076923077 0.0243525061579114
13.1794871794872 0.0246870424460529
13.6666666666667 0.0250084174449682
14.1538461538462 0.025317472003792
14.6410256410256 0.0256149683042287
15.1282051282051 0.0259016046608144
15.6153846153846 0.0261780187794169
16.1025641025641 0.0264447857917398
16.5897435897436 0.0267024495248842
17.0769230769231 0.0269515013969153
17.5641025641026 0.0271924011777871
18.0512820512821 0.02742556947944
18.5384615384615 0.0276513942851538
19.025641025641 0.0278702473252279
19.5128205128205 0.0280824588012418
20 0.0282883485877853
};
%\addlegendentry{ece of ts}
\addplot [semithick, color0]
table {%
1 0.00664009455687951
1.48717948717949 0.00753187032558004
1.97435897435897 0.00871110290121841
2.46153846153846 0.0102352353904734
2.94871794871795 0.0116577755787141
3.43589743589744 0.0129082789159978
3.92307692307692 0.0140145700591852
4.41025641025641 0.0150060917107712
4.8974358974359 0.015904922866033
5.38461538461538 0.0167272416717163
5.87179487179487 0.0174851438731292
6.35897435897436 0.0181879104084556
6.84615384615385 0.0188428365230104
7.33333333333333 0.0194557784460004
7.82051282051282 0.0200315225724321
8.30769230769231 0.020574041546187
8.7948717948718 0.0210866764785656
9.28205128205128 0.021572269659873
9.76923076923077 0.0220332632450907
10.2564102564103 0.0224717740230686
10.7435897435897 0.0228896510010289
11.2307692307692 0.0232885204237805
11.7179487179487 0.0236698214380084
12.2051282051282 0.0240348346872564
12.6923076923077 0.024384705488321
13.1794871794872 0.0247204627963225
13.6666666666667 0.0250430348724926
14.1538461538462 0.0253532623259684
14.6410256410256 0.0256519090547121
15.1282051282051 0.0259396714921995
15.6153846153846 0.0262171864570712
16.1025641025641 0.0264850378776705
16.5897435897436 0.0267437625669575
17.0769230769231 0.0269938552113207
17.5641025641026 0.0272357727091466
18.0512820512821 0.0274699379525404
18.5384615384615 0.0276967431324786
19.025641025641 0.0279165526490819
19.5128205128205 0.02812970568573
20 0.0283365184779806
};
%\addlegendentry{ece of ec}
\end{axis}

\end{tikzpicture}


==> rho_10/logit_teacher_rho_10_ece_difference.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figheight,
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \alpha\)},
xmajorgrids,
xmin=-1.95, xmax=40.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle ECE(EC) - ECE(TS)\)},
ymajorgrids,
ymin=-1.62815369038989e-06, ymax=5.054122561845e-05,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
0 7.43181732739198e-07
1 1.07992799192481e-06
2 1.66240640713834e-06
3 2.67844059278696e-06
4 3.92675452749042e-06
5 5.28938336354784e-06
6 6.72188216423002e-06
7 8.19412388099357e-06
8 9.69153105707943e-06
9 1.12003549312713e-05
10 1.27127872753888e-05
11 1.4221115869878e-05
12 1.57215172410276e-05
13 1.72101176960232e-05
14 1.86822342041794e-05
15 2.01354308615453e-05
16 2.15681274968044e-05
17 2.29804023801107e-05
18 2.43704412149354e-05
19 2.57360485620313e-05
20 2.70802213737376e-05
21 2.83947600103265e-05
22 2.96885580197935e-05
23 3.09563707746735e-05
24 3.21993304096303e-05
25 3.34203502696043e-05
26 3.46174275244401e-05
27 3.57903221763801e-05
28 3.69407504834593e-05
29 3.8066831385089e-05
30 3.91676776543178e-05
31 4.02520859307011e-05
32 4.13130420732905e-05
33 4.23538144054478e-05
34 4.33715313595401e-05
35 4.4368473100409e-05
36 4.53488473247908e-05
37 4.6305323854013e-05
38 4.72468844882681e-05
39 4.81698901953209e-05
};
\end{axis}

\end{tikzpicture}

